SureMap: Simultaneous Mean Estimation for Single-Task and Multi-Task Disaggregated Evaluation

Disaggregated evaluation -- estimation of performance of a machine learning model on different subpopulations -- is a core task when assessing performance and group-fairness of AI systems. A key challenge is that evaluation data is scarce, and subpopulations arising from intersections of attributes (e.g., race, sex, age) are often tiny. Today, it is common for multiple clients to procure the same AI model from a model developer, and the task of disaggregated evaluation is faced by each customer individually. This gives rise to what we call the multi-task disaggregated evaluation problem, wherein multiple clients seek to conduct a disaggregated evaluation of a given model in their own data setting (task). In this work we develop a disaggregated evaluation method called SureMap that has high estimation accuracy for both multi-task and single-task disaggregated evaluations of blackbox models. SureMap's efficiency gains come from (1) transforming the problem into structured simultaneous Gaussian mean estimation and (2) incorporating external data, e.g., from the AI system creator or from their other clients. Our method combines maximum a posteriori (MAP) estimation using a well-chosen prior together with cross-validation-free tuning via Stein's unbiased risk estimate (SURE). We evaluate SureMap on disaggregated evaluation tasks in multiple domains, observing significant accuracy improvements over several strong competitors.

==> multi.tex <==

\subsection{How to set the multi-task center}\label{app:mt}

In the single-task case we set the prior mean $\@\theta=\*0_d$;
this can also be done in the multi-task setting.
Alternatively, we can use multi-task data to construct estimator $\@{\hat\theta}$ of some true underlying multi-task mean $\@\theta$ and substitute the former for $\@\theta$;
for simplicity we will restrict to the ourselves to {\em linear} estimators $\@{\hat\theta}=\sum_{t=1}^T\*M_t\*y_t$, where the matrices $\*M_1,\dots,\*M_T$ are independent of $\*y_1,\dots,\*y_T$.
To determine these matrices, we will assign them some parametric form and set those parameters by minimizing the sum of the $\@\Sigma_t^{-1}$-weighted risks across tasks, as estimated by SURE:
\begin{align}
	\begin{split}
		\sum_{t=1}^T\E_t\|\@{\hat\mu}_{\@{\hat\theta},\@\Lambda}^\textrm{MAP}(\*y_t)-\@\mu_t\|_{\@\Sigma_t^{-1}}^2
		&=\sum_{t=1}^T\E_t\left(\|\@{\hat\mu}_{\@{\hat\theta},\@\Lambda}^\textrm{MAP}(\*y_t)-\*y_t\|_{\@\Sigma_t^{-1}}^2-d+2\nabla_{\*y_t}\cdot\@{\hat\mu}_{\@{\hat\theta},\@\Lambda}^\textrm{MAP}(\*y_t)\right)\\
		&=dT+\sum_{t=1}^T\E_t\|\*A_t(\@{\hat\theta}-\*y_t)\|_{\@\Sigma_t^{-1}}^2+2\Tr(\*A_t\*M_t-\*A_t)
	\end{split}
\end{align}
for $\*A_t=(\@\Lambda^{-1}+\@\Sigma_t^{-1})^{-1}\@\Lambda^{-1}$, i.e. $\@{\hat\mu}_{\@{\hat\theta},\@\Lambda}^\textrm{MAP}(\*y_t)=\*y_t+\*A_t(\@{\hat\theta}-\*y_t)=\*y_t-\*A_t(\*y_t-\sum_{s=1}^T\*M_s\*y_s)$.

\subsubsection{SureSolve}

This approach sets the prior mean by finding the $\@\theta$ that minimizes the above SURE objective, which is equivalent to solving an overconstrained linear system:
\begin{equation}
	\@{\hat\theta}
	=dT+\argmin_{\@\theta\in\R^d}\sum_{t=1}^T\|\*A_t(\@\theta-\*y_t)\|_{\@\Sigma_t^{-1}}^2-2\Tr(\*A_t)
	=\left(\sum_{t=1}^T\*A_t^\top\@\Sigma_t^{-1}\*A_t\right)^{-1}\sum_{t=1}^T\*A_t^\top\@\Sigma_t^{-1}\*A_t\*y_t
\end{equation}
Note that this estimator can be expressed in the desired linear form $\@{\hat\theta}=\sum_{t=1}^T\*M_t\*y_t$, with the matrices $\*M_t=\left(\sum_{s=1}^T\*A_s^\top\@\Sigma_s^{-1}\*A_s\right)^{-1}\*A_t^\top\@\Sigma_t^{-1}\*A_t$ depending on the parameters determining $\@\Lambda$.

\subsubsection{MetaMap}

Alternatively, if we assume the prior is correct for some $\@\theta$ and $\@\Lambda$, i.e. $\*y_t\sim\N(\@\theta,\@\Lambda+\@\Sigma_t)$, then a natural estimator to use for $\@\theta$ given a fixed $\@\Lambda$ is a MAP estimator of $\@{\hat\theta}_\@\Gamma$ with prior $\N(\*0_d,\@\Gamma)$ for some covariance $\@\Gamma$.
Define $\@\Sigma_\@\Lambda=(\sum_{t=1}^T(\@\Lambda+\@\Sigma_t)^{-1})^{-1}$ and note that
$\*y_\@\Lambda=\@\Sigma_\@\Lambda\sum_{t=1}^T(\@\Lambda+\@\Sigma_t)^{-1}\*y_t$ is distributed as $\N(\@\theta,T\@\Sigma_\@\Lambda)$.
Then the MAP estimator of $\@\theta$
\begin{equation}
	\@{\hat\theta}_\@\Gamma
	=\left(T\@\Gamma^{-1}+\@\Sigma_\@\Lambda^{-1}\right)^{-1}\@\Sigma_\@\Lambda^{-1}\*y_\@\Lambda
	=\sum_{t=1}^T\left(T\@\Gamma^{-1}+\@\Sigma_\@\Lambda^{-1}\right)^{-1}(\@\Lambda+\@\Sigma_t)^{-1}\*y_t
\end{equation}
has the necessary form $\@{\hat\theta}=\sum_{t=1}^T\*M_t\*y_t$ for $\*M_t=(T\@\Gamma^{-1}+\@\Sigma_\@\Lambda^{-1})^{-1}(\@\Lambda+\@\Sigma_t)^{-1}$.
In this case the matrices depend on both $\@\Lambda$ and $\@\Gamma$, i.e. the covariance matrices of the prior {\em and} the meta-prior.

\subsection{Optimization}

In both cases above we have the SURE objective
\begin{equation}
	dT+\sum_{t=1}^T\E_t\left\|\*A_t\left(\*y_t-\sum_{s=1}^T\*M_s\*y_s\right)\right\|_{\@\Sigma_t^{-1}}^2+2\Tr(\*A_t\*M_t-\*A_t)
\end{equation}
The tuning parameters are the coefficients $\tau_1^2,\dots,\tau_k^2$ used to define the prior covariance $\@\Lambda=\sum_{i=1}^k\tau_i^2\*U_i\*U_i^\top$ and, in the second case, the coefficients $\upsilon_1^2,\dots,\upsilon_k^2$ used to define the meta-prior covariance $\@\Gamma=\sum_{i=1}^k\upsilon_i^2\*U_i\*U_i^\top$.
Noting that $\*A_t
=(\@\Lambda+\@\Sigma_t^{-1})^{-1}\@\Lambda^{-1}
=(\*I_d+\@\Lambda\@\Sigma_t^{-1})^{-1}$ and $(\@\Lambda+\@\Sigma_t)^{-1}
=\@\Lambda^{-1}(\*I_d+\@\Sigma_t\@\Lambda^{-1})^{-1}
=\@\Sigma_t^{-1}(\*I_d+\@\Lambda\@\Sigma_t^{-1})^{-1}
=\@\Sigma_t^{-1}\*A_t$, we have the derivative $\partial_i\*A_t
=-\*A_t\*U_i\*U_i^\top\@\Sigma_t^{-1}\*A_t$ w.r.t. $\tau_i^2$, which yields $\partial_i\Tr(\*A_t)
=\Tr(-\*A_t\*U_i\*U_i^\top\@\Sigma_t^{-1}\*A_t)$ and 
\begin{align}
\begin{split}
\partial_i\|\*A_t(\@\theta-\*y_t)\|_{\@\Sigma_t^{-1}}^2
&=2(\@\theta-\*y_t)^\top\*A_t^\top\@\Sigma_t^{-1}\partial_i\*A_t(\@\theta-\*y_t)\\
&=-2(\@\theta-\*y_t)^\top\*A_t^\top\@\Sigma_t^{-1}\*A_t\*U_i\*U_i^\top\@\Sigma_t^{-1}\*A_t(\@\theta-\*y_t)
\end{split}
\end{align}

\subsubsection{SureSolve}

First note that
\begin{align}
\begin{split}
	\partial_i[\*A_t^\top\@\Sigma_t^{-1}\*A_t]
	=\partial_i[\@\Sigma_t^{-1}\*A_t^2]
	&=\@\Sigma_t^{-1}(\*A_t\partial_i\*A_t+\partial_i\*A_t\*A_t)\\
	&=-\@\Sigma_t^{-1}(\*A_t^2+\*A_t)\*U_i\*U_i^\top\@\Sigma_t^{-1}(\*A_t^2+\*A_t)
\end{split}
\end{align}
where the first step follows by $\@\Sigma_t^{-1}\*A_t
=\@\Sigma_t^{-1}(\*I_d+\@\Lambda\@\Sigma_t^{-1})^{-1}
=(\*I_d+\@\Sigma_t^{-1}\@\Lambda)^{-1}\@\Sigma_t^{-1}
=\*A_t^\top\@\Sigma_t^{-1}$.
Then for $\*M_t=\left(\sum_{s=1}^T\*A_s^\top\@\Sigma_s^{-1}\*A_s\right)^{-1}\*A_t^\top\@\Sigma_t^{-1}\*A_t$ we have
\begin{align}
\begin{split}
	\partial_i\*M_t
	&=\left(\sum_{s=1}^T\*A_s^\top\@\Sigma_s^{-1}\*A_s\right)^{-1}\partial_i[\*A_t^\top\@\Sigma_t^{-1}\*A_t]-\left(\sum_{s=1}^T\*A_s^\top\@\Sigma_s^{-1}\*A_s\right)^{-1}\sum_{s=1}^T\partial_i[\*A_s^\top\@\Sigma_s^{-1}\*A_s]\*M_t\\
	&=-2\left(\sum_{s=1}^T\*A_s^\top\@\Sigma_s^{-1}\*A_s\right)^{-1}\@\Sigma_t^{-1}(\*A_t^2+\*A_t)\*U_i\*U_i^\top\@\Sigma_t^{-1}(\*A_t^2+\*A_t)\\
	&\quad+2\left(\sum_{s=1}^T\*A_s^\top\@\Sigma_s^{-1}\*A_s\right)^{-1}\sum_{s=1}^T\@\Sigma_s^{-1}(\*A_s^2+\*A_s)\*U_i\*U_i^\top\@\Sigma_s^{-1}(\*A_s^2+\*A_s)\*M_t\\
	&=-2\*B_{i,t}+2\sum_{s=1}^T\*B_{i,s}\*M_t
\end{split}
\end{align}
where $\*B_{i,t}=\left(\sum_{s=1}^T\*A_s^\top\@\Sigma_s^{-1}\*A_s\right)^{-1}\@\Sigma_t^{-1}(\*A_t^2+\*A_t)\*U_i\*U_i^\top\@\Sigma_t^{-1}(\*A_t^2+\*A_t)$.
We can then compute
\begin{align}
\begin{split}
	\partial_i\Tr(\*A_t\*M_t)
	&=-2\Tr\left(\*A_t\left(\*B_{i,t}-\sum_{s=1}^T\*B_{i,s}\*M_t\right)\right)-\Tr(\*A_t\*U_i\*U_i^\top\@\Sigma_t^{-1}\*A_t\*M_t)\\
	&=-2\Tr\left(\*A_t\left(\*B_{i,t}+\left(\*U_i\*U_i^\top\@\Sigma_t^{-1}\*A_t-\sum_{s=1}^T\*B_{i,s}\right)\*M_t\right)\right)
\end{split}
\end{align}
and 
\begin{align}
	\begin{split}
		\partial_i\left\|\*A_t\left(\*y_t-\sum_{s=1}^T\*M_s\*y_s\right)\right\|_{\@\Sigma_t^{-1}}^2
		&=\partial_i\sum_{s=1}^T\sum_{r=1}^T(\*y_t-\*M_s\*y_s)^\top\*A_t^\top\@\Sigma_t^{-1}\*A_t(\*y_t-\*M_r\*y_r)\\
		&=-2\sum_{s=1}^T(\partial_i\*M_s\*y_s)^\top\*A_t^\top\@\Sigma_t^{-1}\*A_t(\*y_t-\@{\hat\theta})\\
		&\quad+2(\*y_t-\@{\hat\theta})^\top\*A_t^\top\@\Sigma_t^{-1}\partial_i\*A_t(\*y_t-\@{\hat\theta})\\
		&=4\sum_{s=1}^T\*y_s^\top\*B_{i,s}^\top\*A_t^\top\@\Sigma_t^{-1}\*A_t(\*y_t-\@{\hat\theta})\\
		&\quad-4\@{\hat\theta}^\top\sum_{s=1}^T\*B_{i,s}^\top\*A_t^\top\@\Sigma_t^{-1}\*A_t(\*y_t-\@{\hat\theta})\\
		&\quad-2(\*y_t-\@{\hat\theta})^\top\*A_t^\top\@\Sigma_t^{-1}\*A_t\*U_i\*U_i^\top\@\Sigma_t^{-1}\*A_t(\*y_t-\@{\hat\theta})\\
		&=4\sum_{s=1}^T(\*y_s-\@{\hat\theta})^\top\*B_{i,s}^\top\*A_t^\top\@\Sigma_t^{-1}\*A_t(\*y_t-\@{\hat\theta})\\
		&\quad-2(\*y_t-\@{\hat\theta})^\top\*A_t^\top\@\Sigma_t^{-1}\*A_t\*U_i\*U_i^\top\@\Sigma_t^{-1}\*A_t(\*y_t-\@{\hat\theta})
	\end{split}
\end{align}


\subsection{MetaMap}

Note that $(\@\Lambda+\@\Sigma_t)^{-1}
=\@\Sigma_t^{-1}(\@\Lambda\@\Sigma_t^{-1}+\*I_d)
=\@\Sigma_t^{-1}\*A_t$ so we can write the matrices representing the estimator as $\*M_t
=(T\@\Gamma^{-1}+\@\Sigma_\@\Lambda^{-1})^{-1}(\@\Lambda+\@\Sigma_t)^{-1}
=(T\@\Gamma^{-1}+\sum_{s=1}^T\@\Sigma_s^{-1}\*A_s)^{-1}\@\Sigma_t^{-1}\*A_t$.
Thus
\begin{align}
\begin{split}
\partial_i\*M_t
&=(T\@\Gamma^{-1}+\@\Sigma_\@\Lambda^{-1})^{-1}\@\Sigma_t^{-1}\partial_i\*A_t-(T\@\Gamma^{-1}+\@\Sigma_\@\Lambda^{-1})^{-1}\sum_{s=1}^T\@\Sigma_s^{-1}\partial_i\*A_s\*M_t\\
&=-\*M_t\*U_i\*U_i^\top\@\Sigma_t^{-1}\*A_t+\sum_{s=1}^T\*M_s\*U_i\*U_i^\top\@\Sigma_s^{-1}\*A_s\*M_t
\end{split}
\end{align}
We can then compute
\begin{align}
\begin{split}
\partial_i\Tr(\*A_t\*M_t)
&=-\Tr(\*A_t(\*M_t\*A_t+\*A_t\*M_t)\*U_i\*U_i^\top\@\Sigma_t^{-1})+\sum_{s=1}^T\Tr(\*A_t\*M_s\*U_i\*U_i^\top\@\Sigma_s^{-1}\*A_s\*M_t)
\end{split}
\end{align}
and
\begin{align}
\begin{split}
\partial_i\left\|\*A_t\left(\*y_t-\sum_{s=1}^T\*M_s\*y_s\right)\right\|_{\@\Sigma_t^{-1}}^2
&=\partial_i\sum_{s=1}^T\sum_{r=1}^T(\*y_t-\*M_s\*y_s)^\top\*A_t^\top\@\Sigma_t^{-1}\*A_t(\*y_t-\*M_r\*y_r)\\
&=-2\sum_{s=1}^T(\partial_i\*M_s\*y_s)^\top\*A_t^\top\@\Sigma_t^{-1}\*A_t(\*y_t-\@{\hat\theta}_\@\Gamma)\\
&\quad+2(\*y_t-\@{\hat\theta}_\@\Gamma)^\top\*A_t^\top\@\Sigma_t^{-1}\partial_i\*A_t(\*y_t-\@{\hat\theta}_\@\Gamma)\\
&=2\sum_{s=1}^T\*y_s^\top(\*M_s\*U_i\*U_i^\top\@\Sigma_s^{-1}\*A_s)^\top\*A_t\@\Sigma_t^{-1}\*A_t(\*y_t-\@{\hat\theta}_\@\Gamma)\\
&\quad-2\sum_{s=1}^T\sum_{r=1}^T\*y_s^\top(\*M_r\*U_i\*U_i^\top\@\Sigma_r^{-1}\*A_r\*M_s)^\top\*A_t\@\Sigma_t^{-1}\*A_t(\*y_t-\@{\hat\theta}_\@\Gamma)\\
&\quad-2(\*y_t-\@{\hat\theta}_\@\Gamma)^\top\*A_t^\top\@\Sigma_t^{-1}\*A_t\*U_i\*U_i^\top\@\Sigma_t^{-1}\*A_t(\*y_t-\@{\hat\theta}_\@\Gamma)\\
&=2\sum_{s=1}^T(\*y_s-\@{\hat\theta}_\@\Gamma)^\top\*A_s^\top\@\Sigma_s^{-1}\*U_i\*U_i^\top\*M_s^\top\*A_t^\top\@\Sigma_t^{-1}\*A_t(\*y_t-\@{\hat\theta}_\@\Gamma)\\
&\quad-2(\*y_t-\@{\hat\theta}_\@\Gamma)^\top\*A_t^\top\@\Sigma_t^{-1}\*A_t\*U_i\*U_i^\top\@\Sigma_t^{-1}\*A_t(\*y_t-\@{\hat\theta}_\@\Gamma)
\end{split}
\end{align}
Lastly, note that $\*M_t=(T\@\Gamma^{-1}+\@\Sigma_\@\Lambda^{-1})^{-1}\@\Sigma_t^{-1}\*A_t=(T\*I_d+\@\Gamma\@\Sigma_\@\Lambda^{-1})^{-1}\@\Gamma\@\Sigma_t^{-1}\*A_t$ and redefine the derivative $\partial_i$ to be w.r.t. $\upsilon_i^2$, so that 
\begin{equation}
	\partial_i\*M_t
	=-(T\*I_d+\@\Gamma\@\Sigma_\@\Lambda^{-1})^{-1}\*U_i\*U_i^\top\@\Sigma_\@\Lambda^{-1}\*M_t+(T\*I_d+\@\Gamma\@\Sigma_\@\Lambda^{-1})^{-1}\*U_i\*U_i^\top\@\Sigma_t^{-1}\*A_t
\end{equation}
Then we have $\partial_i\Tr(\*A_t\*M_t)
=\Tr(\*A_t(T\*I_d+\@\Gamma\@\Sigma_\@\Lambda^{-1})^{-1}\*U_i\*U_i^\top(\@\Sigma_t^{-1}\*A_t-\@\Sigma_\@\Lambda^{-1}\*M_t))$ and
\begin{align}
\begin{split}
	\partial_i&\left\|\*A_t\left(\*y_t-\@{\hat\theta}_\@\Gamma\right)\right\|_{\@\Sigma_t^{-1}}^2\\
	&=-2\sum_{s=1}^T(\partial_i\*M_s\*y_s)^\top\*A_t^\top\@\Sigma_t^{-1}\*A_t(\*y_t-\@{\hat\theta}_\@\Gamma)\\
	&=2\left(\@\Sigma_\@\Lambda^{-1}\@{\hat\theta}_\@\Gamma-\sum_{s=1}^T\@\Sigma_s^{-1}\*A_s\*y_s\right)^\top\*U_i\*U_i^\top(T\*I_d+\@\Gamma\@\Sigma_\@\Lambda^{-1})^{-\top}\*A_t^\top\@\Sigma_t^{-1}\*A_t(\*y_t-\@{\hat\theta}_\@\Gamma)
\end{split}
\end{align}

